Multiparty Session Types, Beyond Duality (Abstract)

Multiparty Session Types (MPST) are a well-established typing discipline for message-passing processes interacting on sessions involving two or more participants. Session typing can ensure desirable properties: absence of communication errors and deadlocks, and protocol conformance. However, existing MPST works provide a subject reduction result that is arguably (and sometimes, surprisingly) restrictive: it only holds for typing contexts with strong duality constraints on the interactions between pairs of participants. Consequently, many "intuitively correct" examples cannot be typed and/or cannot be proved type-safe. We illustrate some of these examples, and discuss the reason for these limitations. Then, we outline a novel MPST typing system that removes these restrictions.

==> eptcsdata.tex <==
\providecommand{\firstpage}{37}
\providecommand{\publicationstatus}{V.T. Vasconcelos and P. Haller (Eds.): Workshop on Programming Language\\ Approaches to Concurrency- and Communication-cEntric Software (PLACES'17)\\
EPTCS 246, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.246.7}{10.4204/EPTCS.246.7}}
\pdfoutput=1

